Des correctifs de securite a la mise a jour

The ever growing software complexity suggests that they will never be bugfree and therefore secure. Software compagnies regulary publish updates. But maybe because of lack of time or care or maybe because stopping application is annoying, such updates are rarely if ever deployed on users' machines. We propose an integrated tool allowing system administrators to deploy critical security updates on the fly on applications running remotly without end-user intervention. Our approach is based on an aspect weaving system, Arachne, that dynamicaly rewrites binary code. Hence updated applications are still running while they are updated. Our second tool Minerve integrates Arachne within the standart updating process: Minerve takes a patch produced by dif and eventually builds a dynamic patch that can later be woven to update the application on the fly. In addition, Minerve allows to consult patches translated in a dedicated language and hence eases auditing tasks.

==> patch.tex <==
% Remember to use the lgrind style

\Head{}
\File{patch.ac}{2004}{6}{15}{16:29}{321}
\L{\LB{\N{1}:}\Tab{3}{\V{ReplaceFunctionCall}_[:}}
\index{input\_userauth\_info\_response}\Proc{input\_userauth\_info\_response}\L{\LB{\N{2}:}\Tab{6}{\K{void}_\V{input\_userauth\_info\_response}(\K{int}_\V{type},_\V{u\_int32\_t}_\V{seq},_\K{void}*_\V{ctxt})_[:_\{}}
\L{\LB{\N{3}:}\Tab{9}{\V{input\_userauth\_info\_response\_new}(\V{type},_\V{seq},_\V{ctxt});}\Tab{60}{\}_:]_:]}}
\L{\LB{\N{4}:}}
\L{\LB{\N{5}:}\Tab{3}{\V{ReplacePointer}_[:}}
\L{\LB{\N{6}:}\Tab{6}{\K{void}*_(\V{input\_userauth\_info\_response})(\K{int},_\V{u\_int32\_t},_\K{void}*)_[:_\{}}
\L{\LB{\N{7}:}\Tab{12}{\K{return}_\&\V{input\_userauth\_info\_response\_new};}\Tab{54}{\}_:]_:]}}


==> patchSource.tex <==
% Remember to use the lgrind style

\Head{}
\File{patchSource.diff}{2004}{6}{16}{10:17}{249}
\L{\LB{_}\Tab{3}{\V{authctxt}\-\!\>\V{postponed}_=_\N{0};}\Tab{30}{\C{}/*_reset_*/\CE{}}}
\L{\LB{_}\Tab{3}{\V{nresp}_=_\V{packet\_get\_int}();}}
\index{if}\Proc{if}\L{\LB{+}\Tab{3}{\K{if}_(\V{nresp}_\>_\N{100})}}
\L{\LB{+}\Tab{6}{\V{fatal}(\S{}\3input\_userauth\_info\_response:_nresp_too_big_\%u\3\SE{},_\V{nresp});}}
\L{\LB{_}\Tab{3}{\K{if}_(\V{nresp}_\>_\N{0})_\{}}
\L{\LB{_}\Tab{6}{\V{response}_=_\V{xmalloc}(\V{nresp}_*_\K{sizeof}(\K{char}*));}}
\L{\LB{_}\Tab{6}{\K{for}_(\V{i}_=_\N{0};_\V{i}_\<_\V{nresp};_\V{i}++)}}

